How to Alleviate Catastrophic Forgetting in LLMs Finetuning? Hierarchical Layer-Wise and Element-Wise Regularization

Large Language Models (LLMs) exhibit strong general language capabilities. However, fine-tuning these models on domain-specific tasks often leads to catastrophic forgetting, where the model overwrites or loses essential knowledge acquired during pretraining. This phenomenon significantly limits the broader applicability of LLMs. To address this challenge, we propose a novel approach to compute the element-wise importance of model parameters crucial for preserving general knowledge during fine-tuning. Our method utilizes a dual-objective optimization strategy: (1) regularization loss based on element-wise parameter importance, which constrains the updates to parameters crucial for general knowledge; (2) cross-entropy loss to adapt to domain-specific tasks. Additionally, we introduce layer-wise coefficients to account for the varying contributions of different layers, dynamically balancing the dual-objective optimization. Extensive experiments on scientific, medical, and physical tasks using GPT-J and LLaMA-3 demonstrate that our approach mitigates catastrophic forgetting while enhancing model adaptability. Compared to previous methods, our solution is approximately 20 times faster and requires only 10-15% of the storage, highlighting the practical efficiency. The code will be released.

==> Tables/casestudy.tex <==
% Table generated by Excel2LaTeX from sheet 'CaseStudy'
\begin{table*}[htbp]
  \centering
  \caption{Case Study in LLaMA}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
          & \multicolumn{3}{c}{LLaMA-3} \\
    \midrule
    Domain & SciQ  & PiQA  & \multicolumn{1}{c}{Medmcqa} \\
    \midrule
    Input & \multicolumn{1}{p{14.5291662216187em}}{"question": "Who proposed the theory of evolution by natural selection?", "distractor3": "Scopes","distractor1": "Linnaeus", "distractor2": "shaw","distractor0": "darwin". } & \multicolumn{1}{p{22em}}{"goal": "How do I ready a guinea pig cage for it's new occupants?", "sol1": "Provide the guinea pig with a cage full of a few inches of bedding made of ripped paper strips, you will also need to supply it with a water bottle and a food dish.", "sol2": "Provide the guinea pig with a cage full of a few inches of bedding made of ripped jeans material, you will also need to supply it with a water bottle and a food dish."} & \multicolumn{1}{p{22em}}{"question":"Which of the following is not true for myelinated nerve fibers:","opa":"Impulse through myelinated fibers is slower than non-myelinated fibers","opb":"Membrane currents are generated at nodes of Ranvier","opc":"Saltatory conduction of impulses is seen","opd":"Local anesthesia is effective only when the nerve is not covered by myelin sheath",} \\
    \midrule
    \textbf{Truth} & "darwin" & "sol1" & \multicolumn{1}{c}{"opa"} \\
    \midrule
    Base  & Answer &       &  \\
    LoRA(B) &       &       &  \\
    LoRA(Seq) &       &       &  \\
    EWC-L &       &       &  \\
    \textbf{Ours} &       &       &  \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:addlabel}%
\end{table*}%

